Noncommutative Geometry and Twisted Little-String Theories

In this thesis we will discuss various aspects of noncommutative geometry and compactified Little-String theories. First we will give an introduction to the use of noncommutative geometry in string theory. Thereafter we will present a proof of the connection between D-brane dynamics and noncommutative geometry. Then we will explain the concept of instantons in noncommutative gauge theories. The last chapters shift the focus to Little-String- and $(2,0)$-theories. We study compactifications of these theories on tori with twists. First we study the case of two coinciding branes in detail. Afterwards we study the case of an arbitrary number of coinciding branes. The main result here is that the moduli spaces of vacua for the twisted compactifications are equal to moduli spaces of instantons on a noncommutative torus. A special case of this is that a large class of gauge theories with $\SUSY{2}$ supersymmetry in D=4 or $\SUSY{4}$ in D=3 has moduli spaces which are moduli spaces of instantons on noncommutative tori.

==> hyperbasics.tex <==
% dummy file

